Search for High-Energy Neutrinos from TDE-like Flares with IceCube

The collected data of IceCube, a cubic kilometre neutrino detector array in the Antarctic ice, reveal a diffuse flux of astrophysical neutrinos. The extragalactic sources of the majority of these neutrinos however have yet to be discovered. Tidal Disruption Events (TDEs), disruption outbursts from black holes that accrete at an enhanced rate, are candidates for being the sources of extragalactic, high-energy neutrinos. Stein et al. (2021) and Reusch et al. (2022) have reported the coincidence of two likely TDEs from supermassive black holes and public IceCube neutrino events (alerts). Further work by van Velzen et al. (2021) identified a third event in coincidence with a high-energy neutrino alert and a $3.7 \sigma$ correlation between a broader set of similar TDE-like flares and IceCube alerts. We conducted a stacking analysis with a 29-flare subset of the TDE-like flares tested by van Velzen et al. This work was done with neutrinos with energies above $\mathcal{O}(100)$ GeV. The resulting p-value of 0.45 is consistent with background. In this contribution, I will discuss the results of the stacking analysis, as well as the impact of using different reconstruction algorithms on the three correlated realtime alerts.

==> acknowledgements.tex <==
\subsection*{Acknowledgements}

\noindent
USA {\textendash} U.S. National Science Foundation-Office of Polar Programs,
U.S. National Science Foundation-Physics Division,
U.S. National Science Foundation-EPSCoR,
Wisconsin Alumni Research Foundation,
Center for High Throughput Computing (CHTC) at the University of Wisconsin{\textendash}Madison,
Open Science Grid (OSG),
Extreme Science and Engineering Discovery Environment (XSEDE),
Frontera computing project at the Texas Advanced Computing Center,
U.S. Department of Energy-National Energy Research Scientific Computing Center,
Particle astrophysics research computing center at the University of Maryland,
Institute for Cyber-Enabled Research at Michigan State University,
and Astroparticle physics computational facility at Marquette University;
Belgium {\textendash} Funds for Scientific Research (FRS-FNRS and FWO),
FWO Odysseus and Big Science programmes,
and Belgian Federal Science Policy Office (Belspo);
Germany {\textendash} Bundesministerium f{\"u}r Bildung und Forschung (BMBF),
Deutsche Forschungsgemeinschaft (DFG),
Helmholtz Alliance for Astroparticle Physics (HAP),
Initiative and Networking Fund of the Helmholtz Association,
Deutsches Elektronen Synchrotron (DESY),
and High Performance Computing cluster of the RWTH Aachen;
Sweden {\textendash} Swedish Research Council,
Swedish Polar Research Secretariat,
Swedish National Infrastructure for Computing (SNIC),
and Knut and Alice Wallenberg Foundation;
Australia {\textendash} Australian Research Council;
Canada {\textendash} Natural Sciences and Engineering Research Council of Canada,
Calcul Qu{\'e}bec, Compute Ontario, Canada Foundation for Innovation, WestGrid, and Compute Canada;
Denmark {\textendash} Villum Fonden and Carlsberg Foundation;
New Zealand {\textendash} Marsden Fund;
Japan {\textendash} Japan Society for Promotion of Science (JSPS)
and Institute for Global Prominent Research (IGPR) of Chiba University;
Korea {\textendash} National Research Foundation of Korea (NRF);
Switzerland {\textendash} Swiss National Science Foundation (SNSF);
United Kingdom {\textendash} Department of Physics, University of Oxford.
